Future Physics Programme of BESIII

There has recently been a dramatic renewal of interest in the subjects of hadron spectroscopy and charm physics. This renaissance has been driven in part by the discovery of a plethora of charmonium-like $XYZ$ states at BESIII and $B$ factories, and the observation of an intriguing proton-antiproton threshold enhancement and the possibly related $X(1835)$ meson state at BESIII, as well as the threshold measurements of charm mesons and charm baryons. We present a detailed survey of the important topics in tau-charm physics and hadron physics that can be further explored at BESIII over the remaining lifetime of BEPCII operation. This survey will help in the optimization of the data-taking plan over the coming years, and provides physics motivation for the possible upgrade of BEPCII to higher luminosity.

==> New_physics/np_summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary and prospects}
\label{sec:summary}

In this chapter, we have shown the \bes3 experiment has great
opportunities to perform searches for NP in a variety of channels, thanks
to its high luminosity, a clean collision environment, and excellent
detector performance.

With the accumulation of large data sets and possible increase of
luminosity and cms energy, as well as an ever-improving understanding
of the detector performance, \bes3 will have great potentail in NP
searches in the coming years.


